A Practical Guide to PID Controller Implementation

How difficult can it be to implement a PID controller? The answer is twofold. Implementing the PID control law is simple and computationally inexpensive. However, this basic form will not work in practical applications. The primary reason for this is the various physical limitations of the actuator. Measurement noise, different implementations depending on the various structures (P, PI, PD or PID), bumpless transfer, and varying sampling interval also result in problems rendering the basic form inoperable. PID implementation is therefore more difficult than meets the eye. This paper introduces a reference implementation of the PID controller which considers these practical issues. It includes pseudo-code, discussion of the implementation choices and simulation of carefully selected, important test cases.

==> code/kontrol.tex <==
% Kristian's personal fork of SIMPLE self-contained PID
% (Please don't remove this file)
%
% Parameters: kp,ki,kd,b,umin,umax,dumin,dumax,Dt,Tf
% Could consider 'a' parameter for efficiency
%
% Filter is Tustin approximation of cascade:
% F(s)=F1)(s)*F1(s), F1(s)=1/(s*Tf+1)
% Remove 'Filter measurement' if filtering outside PID
%
% Leadig letter in names
% x  State variable (must survive between calls)
% D  Time increment (Dy=y-xy)
% d  Derivative (yd approximates derivative of y)
%
% Initialization of states is another matter
% Controller should preferrably run in man or disables while filter converges
%
% Inputs:
% r     Reference (setpoint)
% y     Measurement
% uff   Feed-forward control signal (to be included in u)
% um    Output if mode==MAN (uff ignored)
% ut    Signal to be tracked if mode=="TRACK"
% mode  Decidess mode based on macros:
%          0b00: DIS
%          0b01: MAN
%          0b10: AUTO
%          0b11: TRACK

function u=pid(r,y,uff,um,ut,mode)
  % Rate limits 
  usmin=max(umin,xus+Dt*dumin)
  usmax=min(umax,xus+Dt*dumax)

  % Filter measurement
  a=Dt/(Tf+0.5*Dt) % Update only when Dt or Tf change
  xy1=xy1+a*(y-xy1)
  xy2=xy2+a*(xy1-xy2)
  y=xy2

  % Approximate derivative
  Dy=y-xy
  dy=Dy/Dt

  %  Update control signal
  if mode==TRACK
    % Tracking mode
    xu=ut
  end
  if mode==MAN
    % Manual mode
    u=um
    % Output disabled
  elseif mode==DIS
    u=NaN
  elseif ki==0 % AUTO (or TRACK)
    % Position form (P,PD,D)
    u=u0+kp*(b*r-y)-kd*dy+uff
  else % AUTO or TRACK
    % Incremental form
    Dr=r-xr
    Ddy=dy-xdy

    % Control signal increments
    Dup=kp*(b*Dr-Dy)
    Dui=ki*Dt*(r-y)
    Dud=-kd*Ddy
    Duff=uff-xuff

    % Nominal and saturated control signal
    u=xu+Dup+Dui+Dud+Duff
    us=max(min(us,usmax),usmin)

    % Integrator anti-wimdup
    if Dui*(u-us)>0
      %u=u-Dui
      u=u-sign(u-us)*min(abs(Dui),abs(u-us))
    end
  end

  % Saturate control signal
  xu=u
  u=max(min(u,usmax),usmin)

  % Update remaining states
  xus=u
  xr=r
  xy=y
  xdy=dy
  xuff=uff
  xy=y
end
